Convergence analysis of a solver for the linear Poisson--Boltzmann model

This work investigates the convergence of a domain decomposition method for the Poisson-Boltzmann model that can be formulated as an interior-exterior transmission problem. To study its convergence, we introduce an interior-exterior constant providing an upper bound of the $L^2$ norm of any harmonic function in the interior, and establish a spectral equivalence for related Dirichlet-to-Neumann operators to estimate the spectrum of interior-exterior iteration operator. This analysis is nontrivial due to the unboundedness of the exterior subdomain, which distinguishes it from the classical analysis of the Schwarz alternating method with nonoverlapping bounded subdomains. It is proved that for the linear Poisson-Boltzmann solvent model in reality, the convergence of interior-exterior iteration is ensured when the relaxation parameter lies between 0 and 2. This convergence result interprets the good performance of ddLPB method developed in [SIAM Journal on Scientific Computing, 41 (2019), pp. B320-B350] where the relaxation parameter is set to 1. Numerical simulations are conducted to verify our convergence analysis and to investigate the optimal relaxation parameter for the interior-exterior iteration.

==> tmp_Conv_IntExt_202412_header.tex <==
\title{Convergence analysis of a solver for the linear Poisson--Boltzmann model\thanks{Submitted in December, 2024.}}

% \author{
% Xuanyu Liu
% \thanks{National Key Laboratory of Electromagnetic Space Security, Southwest China Research Institute of Electronic Equipment, Chengdu, China (\email{xyuliu0@gmail.com}).}
\author{
Xuanyu Liu
\thanks{School of Mathematical Sciences, Beijing Normal University, Beijing, China (\email{xyliu9535@mail.bnu\\.edu.cn}).}
\and
Yvon Maday
\thanks{Sorbonne Universit\'e, CNRS, Universit\'e Paris Cit\'e, Laboratoire Jacques-Louis Lions (LJLL), F-75005 Paris, France
(\email{yvon.maday@sorbonne-universite.fr}).}
\and
Chaoyu Quan
\thanks{Division of Mathematics, School of Science and Engineering, The Chinese University of Hong Kong, Shenzhen, 518172, Guangdong, China
(\email{quanchaoyu@cuhk.edu.cn}).}
\and
Hui Zhang
\thanks{Department of Applied Mathematics, Xi'an Jiaotong-Liverpool University, Suzhou, Jiangsu, China (\email{hui.zhang@xjtlu.edu.cn}).}
}


% Custom SIAM macro to insert headers
\headers{Convergence of interior-exterior domain decomposition method}{X. Liu, Y. Maday, C. Quan and H. Zhang}

